Improved Bounds on Information Dissemination by Manhattan Random Waypoint Model

With the popularity of portable wireless devices it is important to model and predict how information or contagions spread by natural human mobility -- for understanding the spreading of deadly infectious diseases and for improving delay tolerant communication schemes. Formally, we model this problem by considering $M$ moving agents, where each agent initially carries a \emph{distinct} bit of information. When two agents are at the same location or in close proximity to one another, they share all their information with each other. We would like to know the time it takes until all bits of information reach all agents, called the \textit{flood time}, and how it depends on the way agents move, the size and shape of the network and the number of agents moving in the network. We provide rigorous analysis for the \MRWP model (which takes paths with minimum number of turns), a convenient model used previously to analyze mobile agents, and find that with high probability the flood time is bounded by $O\big(N\log M\lceil(N/M) \log(NM)\rceil\big)$, where $M$ agents move on an $N\times N$ grid. In addition to extensive simulations, we use a data set of taxi trajectories to show that our method can successfully predict flood times in both experimental settings and the real world.

==> bike.tex <==
%bike data 


\begin{table}[!tbh]
\centering
\caption{Number of casual (temporary bike riders) and
regular (long-term subscribers) trips for each city.}
\label{table:bike_data_stats}
\begin{tabular}{|c | c c c|}
 \hline
 \textbf{City} & \textbf{\#Casual} & \textbf{\#Regular} & \textbf{\#Total} \\
 \hline
 New York City & 1.51 M & 12.34 M & 13.81 M \\
 Washington DC & 0.85 M & 3.13 M & 3.98 M \\
 Boston & 0.25 M & 1.15 M & 1.40 M \\
 Chicago & 1.18 M & 3.97 M &  5.15 M \\
 \hline
\end{tabular}
\end{table}


\begin{figure*} %[!tbh]
\centering
\includegraphics[width=\linewidth]{s03_cities.pdf}
\caption{Probability distribution of selecting the next destination based on the distance from the current location. (top) Casual bikers have a higher percentage of mid-range popular destinations (highlighted) that can be treated as a uniform distribution. (bottom) The end tail of both distributions look like a \Levy walk distribution with different values of $\alpha$.}
\label{fig:validation}
\end{figure*}



Our work is motivated by the available bike rental records provided by bike sharing program
in $4$ major US cities, namely New York City \cite{NYCBikeData}, Washington DC \cite{DCBikeData}, Boston \cite{BostonBikeData} and Chicago \cite{ChicagoBikeData}. We are using the last $12$ months of rental records in each city, which includes the check-out and check-in bike stations and timestamps of each trip along with the membership type of the customer renting a bike. There are two types of customers: (1) \emph{casual} customers who use temporary passes to ride the bikes and
(2) \emph{regular} customers who subscribe to long-term (monthly or annual) plans. Table
\ref{table:bike_data_stats} shows the number of records for each type of customers in the $4$ cities.
We also plot the distribution of travel distances from the rental records in Figure~\ref{fig:validation}.
Casual and regular bikers show distinctively different mobility patterns.
While regular bikers show heavy concentration on small distances, casual bikers
tend to have wider peaks at longer distances, as it is apparent by the highlighted areas in the top 4 plots in figure \ref{fig:validation}.
The percentage of bins having at least $1/4$ of the maximum probability is on average $27.9\%$ for
casual bikers while it is only $14.65\%$ for regular bikers.
Casual bikers also show a fat-tailed distribution of destinations,
apparent in the 4 plots at the bottom of figure \ref{fig:validation}.

The distribution for casual bikers can be divided into three separate regimes: short distances that comprise a very small number of records; medium distances that account for most trips, and among these the probability distribution is roughly uniform; and long distances that are rare, but are much longer than the distance in the medium range.
The probabilities in the long distance range shows an exponentially fast decrease as distance increases.

